(U)NFV: Supervised and Unsupervised Neural Finite Volume Methods for Solving Hyperbolic PDEs

We introduce (U)NFV, a modular neural network architecture that generalizes classical finite volume (FV) methods for solving hyperbolic conservation laws. Hyperbolic partial differential equations (PDEs) are challenging to solve, particularly conservation laws whose physically relevant solutions contain shocks and discontinuities. FV methods are widely used for their mathematical properties: convergence to entropy solutions, flow conservation, or total variation diminishing, but often lack accuracy and flexibility in complex settings. Neural Finite Volume addresses these limitations by learning update rules over extended spatial and temporal stencils while preserving conservation structure. It supports both supervised training on solution data (NFV) and unsupervised training via weak-form residual loss (UNFV). Applied to first-order conservation laws, (U)NFV achieves up to 10x lower error than Godunov's method, outperforms ENO/WENO, and rivals discontinuous Galerkin solvers with far less complexity. On traffic modeling problems, both from PDEs and from experimental highway data, (U)NFV captures nonlinear wave dynamics with significantly higher fidelity and scalability than traditional FV approaches.

==> burgers_godunov.tex <==
-0.45774102210998535
-0.47943851351737976
-0.47944551706314087
-0.48079714179039
-0.4836008846759796
-0.48789024353027344
-0.4935864806175232
-0.5004717707633972
-0.5081896185874939
-0.5162827372550964
-0.524261474609375
-0.5316821336746216
-0.5382095575332642
-0.5436459183692932
-0.5479251742362976
-0.5510857105255127
-0.5532329678535461
-0.5545059442520142
-0.5550516247749329
-0.5550099611282349
-0.5545051097869873
-0.5536442399024963
-0.5525172352790833
-0.5512006878852844
-0.549760103225708
-0.54825359582901
-0.5467346906661987
-0.5452549457550049
-0.543864905834198
-0.5426169633865356
-0.541565477848053
-0.5407683849334717
-0.5402880311012268
-0.5401911735534668
-0.5405497550964355
-0.5414406061172485
-0.5429450273513794
-0.5451481342315674
-0.5481379628181458
-0.5520070195198059
-0.5568524599075317
-0.5627801418304443
-0.5699069499969482
-0.5783600211143494
-0.5882648825645447
-0.5997158288955688
-0.612724781036377
-0.6271573305130005
-0.6426756381988525
-0.6587234139442444
-0.6745782494544983
-0.6894657015800476
-0.7026978135108948
-0.7137826681137085
-0.7224709987640381
-0.7287393808364868
-0.7327324151992798
-0.734694242477417
-0.734909176826477
-0.7336596250534058
-0.7312024831771851
-0.7277581691741943
-0.7235094904899597
-0.7186033725738525
-0.7131569385528564
-0.7072619795799255
-0.7009904384613037
-0.6943991780281067
-0.6875326037406921
-0.6804261207580566
-0.6731081604957581
-0.6656022071838379
-0.6579273343086243
-0.6500999331474304
-0.6421336531639099
-0.6340402364730835
-0.6258305907249451
-0.6175135970115662
-0.6090975403785706
-0.6005899906158447
-0.5919974446296692
-0.5833262205123901
-0.5745815634727478
-0.565768837928772
-0.5568927526473999
-0.5479573011398315
-0.5389665961265564
-0.5299242734909058
-0.5208334922790527
-0.5116972923278809
-0.5025185346603394
-0.4932998716831207
-0.48404353857040405
-0.4747517704963684
-0.46542659401893616
-0.4560699164867401
-0.44668352603912354
-0.4372687339782715
-0.4278271794319153
-0.4183601438999176
-0.40886878967285156
-0.39935430884361267
-0.3898176848888397
-0.3802599012851715
-0.3706817328929901
-0.3610839247703552
-0.35146719217300415
-0.34183233976364136
-0.3321796655654907
-0.3225097060203552
-0.3128229081630707
-0.30311962962150574
-0.2934001088142395
-0.2836645245552063
-0.27391350269317627
-0.26414796710014343
-0.2543729543685913
-0.24461019039154053
-0.2349601536989212
-0.22590012848377228
-0.2197335809469223
-0.22702603042125702
-0.28283077478408813
-0.4228406846523285
-0.5822409391403198
-0.6783977150917053
-0.7177808284759521
-0.7310693264007568
-0.7351173758506775
-0.7362599968910217
-0.7365548610687256
-0.7366196513175964
-0.736627995967865
-0.7366251349449158
-0.7366217374801636
-0.736619770526886
-0.7366188764572144
-0.7366185188293457
-0.736618161201477
-0.7366177439689636
-0.736617386341095
-0.7366170287132263
-0.7366166114807129
-0.7366162538528442
-0.7366158962249756
-0.7366154789924622
-0.7366151213645935
-0.7366147637367249
-0.7366143465042114
-0.7366139888763428
-0.7366136312484741
-0.7366132140159607
-0.736612856388092
-0.7366124987602234
-0.73661208152771
-0.7366117238998413
-0.7366113662719727
-0.7366109490394592
-0.7366105914115906
-0.7366102337837219
-0.7366098165512085
-0.7366094589233398
-0.7366091012954712
-0.7366086840629578
-0.7366083264350891
-0.7366079688072205
-0.736607551574707
-0.7366071939468384
-0.7366068363189697
-0.7366064190864563
-0.7366060614585876
-0.736605703830719
-0.7366052865982056
-0.7366049289703369
-0.7366045713424683
-0.7366041541099548
-0.7366037964820862
-0.7366034388542175
-0.7366030216217041
-0.7366026639938354
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> burgers_lax_hopf.tex <==
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.46310532093048096
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5643375515937805
-0.5558617115020752
-0.5458416938781738
-0.5358407497406006
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.573819100856781
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6669842600822449
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.785688042640686
-0.7763025760650635
-0.7662825584411621
-0.7562625408172607
-0.7462424635887146
-0.7362224459648132
-0.7262023687362671
-0.7161823511123657
-0.7061623334884644
-0.6961422562599182
-0.6861222386360168
-0.6761022210121155
-0.6660821437835693
-0.656062126159668
-0.6460420489311218
-0.6360220313072205
-0.6260020136833191
-0.615981936454773
-0.6059619188308716
-0.5959419012069702
-0.5859218239784241
-0.5759018063545227
-0.5658817291259766
-0.5558617115020752
-0.5458416938781738
-0.5358216166496277
-0.5258015990257263
-0.515781581401825
-0.5057615041732788
-0.49574148654937744
-0.4857214391231537
-0.47570139169692993
-0.4656813442707062
-0.4556613266468048
-0.44564127922058105
-0.4356212317943573
-0.42560118436813354
-0.4155811667442322
-0.4055611193180084
-0.39554107189178467
-0.3855210244655609
-0.37550100684165955
-0.3654809594154358
-0.35546091198921204
-0.3454408645629883
-0.3354208469390869
-0.32540079951286316
-0.3153807520866394
-0.30536070466041565
-0.2953406870365143
-0.2853206396102905
-0.2753005921840668
-0.265280544757843
-0.25526052713394165
-0.2452404797077179
-0.23522043228149414
-0.22520039975643158
-0.21518035233020782
-0.20516031980514526
-0.1951402723789215
-0.18512023985385895
-0.1751001924276352
-0.16508015990257263
-0.5342023372650146
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> burgers_ours.tex <==
-0.45774102210998535
-0.4582466781139374
-0.4558110237121582
-0.4572593569755554
-0.45728600025177
-0.4553866982460022
-0.4538269639015198
-0.4621604382991791
-0.5089184641838074
-0.5654846429824829
-0.5688460469245911
-0.5586079359054565
-0.5606938600540161
-0.5655419826507568
-0.5664201378822327
-0.5646724700927734
-0.5644850134849548
-0.5655477643013
-0.5663246512413025
-0.566415548324585
-0.5656936168670654
-0.5637683868408203
-0.5602989196777344
-0.5554412603378296
-0.5497300624847412
-0.5438209772109985
-0.5384002327919006
-0.5341664552688599
-0.5316975116729736
-0.5311172604560852
-0.5317673087120056
-0.5324462056159973
-0.5323379039764404
-0.5316481590270996
-0.531154215335846
-0.5312881469726562
-0.5317276120185852
-0.5317777991294861
-0.5306835770606995
-0.5283282995223999
-0.5269124507904053
-0.5316675305366516
-0.5538604855537415
-0.5894404649734497
-0.6051663756370544
-0.6012213826179504
-0.5944682955741882
-0.5921649932861328
-0.5907291173934937
-0.6257917881011963
-0.7509161233901978
-0.7776041030883789
-0.7762619256973267
-0.7833755016326904
-0.7850922346115112
-0.7933224439620972
-0.7922765612602234
-0.7940557599067688
-0.7906887531280518
-0.7874458432197571
-0.7816678285598755
-0.775099515914917
-0.7676545977592468
-0.7593526244163513
-0.7508342266082764
-0.7417188286781311
-0.7325276136398315
-0.7230558395385742
-0.7134658694267273
-0.7037999033927917
-0.6940213441848755
-0.6842177510261536
-0.6743701696395874
-0.6644889116287231
-0.6545915007591248
-0.6446775794029236
-0.6347544193267822
-0.6248252391815186
-0.6148918867111206
-0.60495525598526
-0.5950173139572144
-0.5850785374641418
-0.5751399397850037
-0.5652014017105103
-0.5552634596824646
-0.5453248620033264
-0.5353848934173584
-0.5254440903663635
-0.5155029296875
-0.5055606961250305
-0.49561694264411926
-0.48567184805870056
-0.4757240414619446
-0.46577394008636475
-0.45582157373428345
-0.44586601853370667
-0.4359075129032135
-0.4259457588195801
-0.41598063707351685
-0.40601176023483276
-0.3960387408733368
-0.3860625922679901
-0.37608230113983154
-0.3660980463027954
-0.3561100959777832
-0.34611833095550537
-0.33612316846847534
-0.3261245787143707
-0.3161216378211975
-0.30611535906791687
-0.2961060404777527
-0.28609392046928406
-0.2760770916938782
-0.26606103777885437
-0.256033718585968
-0.24602270126342773
-0.23596981167793274
-0.2259826362133026
-0.21598957479000092
-0.20588037371635437
-0.19635246694087982
-0.1793651431798935
-0.17934225499629974
-0.16819153726100922
-0.5640231370925903
-0.7452517747879028
-0.732900857925415
-0.7360450029373169
-0.7342157959938049
-0.7375803589820862
-0.7362714409828186
-0.73682701587677
-0.7364663481712341
-0.7366650700569153
-0.7365705370903015
-0.7366182208061218
-0.7365930676460266
-0.7366061210632324
-0.7365995049476624
-0.7366030812263489
-0.7366015911102295
-0.7366019487380981
-0.7366012334823608
-0.7366016507148743
-0.7366024851799011
-0.7366016507148743
-0.7366018295288086
-0.7366015315055847
-0.736601710319519
-0.7366015911102295
-0.7366019487380981
-0.736602246761322
-0.7366021275520325
-0.736602246761322
-0.7366021871566772
-0.7366020679473877
-0.7366021275520325
-0.7366020679473877
-0.7366021275520325
-0.7366020083427429
-0.7366020679473877
-0.7366021275520325
-0.7366021871566772
-0.7366021871566772
-0.7366015911102295
-0.7366018295288086
-0.7366017699241638
-0.7366019487380981
-0.7366019487380981
-0.7366015315055847
-0.7366015315055847
-0.7366018295288086
-0.7366018891334534
-0.7366014122962952
-0.736601710319519
-0.7366017699241638
-0.7366018295288086
-0.7366017699241638
-0.736601710319519
-0.7366019487380981
-0.7366019487380981
-0.7366019487380981
-0.7366019487380981
-0.7366020679473877
-0.7366020679473877
-0.7366021871566772
-0.7366021871566772
-0.7366023063659668
-0.7366021871566772
-0.7366023659706116
-0.7366021275520325
-0.7366020679473877
-0.7366021871566772
-0.7366024255752563
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> greenshield.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 96, 96, 0},
{0, -, 100, 100, 100, 90, 90, 0},
{0, 0, -, 100, 59, 70, 70, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 38, 100, -, 70, 70, 0},
{4, 10, 30, 100, 30, -, 92, 0},
{4, 10, 30, 100, 30, 8, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> ic_burgers_teaser.tex <==
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.6107083559036255
0.550076961517334
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.6019201278686523
-0.5718241333961487
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.9517066478729248
0.8644030690193176
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7943650484085083
-0.7699007987976074
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3050805330276489
-0.3242832124233246
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6891342401504517
-0.6546775102615356
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.7712304592132568
0.732668936252594
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.3751441240310669
0.33144888281822205
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.4987609386444092
-0.5124931931495667
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795
-0.7734057903289795


==> triangular.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 63, 60, 0},
{0, -, 100, 100, 100, 47, 47, 0},
{0, 0, -, 100, 88, 43, 43, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 9, 100, -, 43, 42, 0},
{37, 53, 57, 100, 57, -, 32, 0},
{40, 53, 57, 100, 58, 68, -, 1},
{100, 100, 100, 100, 100, 100, 99, -},
}

==> triangular_godunov.tex <==
0.5
0.522359311580658
0.5170860290527344
0.5124228596687317
0.5085509419441223
0.5055426955223083
0.5033642053604126
0.5019003748893738
0.5009922981262207
0.5004753470420837
0.5002070665359497
0.5000813603401184
0.5000286102294922
0.5000091195106506
0.5000029802322388
0.5000014901161194
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999919533729553
0.4999970495700836
0.49998727440834045
0.49995148181915283
0.4998399317264557
0.4995376467704773
0.498814195394516
0.4972652494907379
0.49426791071891785
0.48898279666900635
0.4804314374923706
0.46765968203544617
0.44996175169944763
0.4271068274974823
0.3994935154914856
0.3681723177433014
0.33471614122390747
0.3009694218635559
0.26874515414237976
0.23955009877681732
0.21440239250659943
0.19377006590366364
0.17762167751789093
0.16555482149124146
0.15695945918560028
0.15117976069450378
0.14764992892742157
0.14599139988422394
0.14606407284736633
0.14796452224254608
0.15196819603443146
0.6329306960105896
0.832298994064331
0.8103061318397522
0.7833358645439148
0.751939058303833
0.7171923518180847
0.6807041168212891
0.6444272398948669
0.6103649139404297
0.5802430510520935
0.5552323460578918
0.5358008742332458
0.5217296481132507
0.5122743844985962
0.5064087510108948
0.5030691027641296
0.5013361573219299
0.5005232095718384
0.500182032585144
0.5000554919242859
0.5000147223472595
0.5000036954879761
0.5000012516975403
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999916553497314
0.4999966621398926
0.49998533725738525
0.4999437928199768
0.49981430172920227
0.4994634687900543
0.49862390756607056
0.49682629108428955
0.4933478832244873
0.48721450567245483
0.4772907793521881
0.46246930956840515
0.4419310688972473
0.4154081344604492
0.38336315751075745
0.3470152020454407
0.3081895411014557
0.2690267562866211
0.23163074254989624
0.19775012135505676
0.1685665100812912
0.14462335407733917
0.12588536739349365
0.11188939958810806
0.10193801671266556
0.09529423713684082
0.09134983271360397
0.0897504910826683
0.09046439826488495
0.09377995133399963
0.1002223864197731
0.45995795726776123
0.7882918119430542
0.7691566944122314
0.7457603216171265
0.71852707862854
0.688388466835022
0.656739354133606
0.6252734065055847
0.5957285761833191
0.5696013569831848
0.5479074716567993
0.5310528874397278
0.5188477635383606
0.510646402835846
0.5055585503578186
0.5026618838310242
0.5011587738990784
0.5004538297653198
0.5001579523086548
0.5000482201576233
0.500012993812561
0.5000033378601074
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.4999992847442627
0.4999975860118866
0.4999898374080658
0.499961256980896
0.49987220764160156
0.49963104724884033
0.49905380606651306
0.4978179335594177
0.4954265058040619
0.4912097752094269
0.48438704013824463
0.4741970896720886
0.4600767195224762
0.44184184074401855
0.4198104739189148
0.3948206901550293
0.3681275248527527
0.3412024676799774
0.3154921531677246
0.29219868779182434
0.272134393453598
0.2556723952293396
0.2427864521741867
0.23315201699733734
0.22627294063568115
0.22160401940345764
0.2186499387025833
0.21703168749809265
0.2165188491344452
0.2170286327600479
0.21859443187713623
0.22130979597568512
0.22525833547115326
0.2304464429616928
0.23675602674484253
0.24393151700496674
0.2516043186187744
0.25934723019599915
0.26674219965934753
0.2734425961971283
0.2792142927646637
0.28394943475723267
0.2876543402671814
0.2904185950756073
0.29237478971481323
0.29365628957748413
0.2943587303161621
0.2945087254047394
0.2940457761287689
0.2928226590156555
0.29063063859939575
0.2872483432292938
0.2825080454349518
0.2763609290122986
0.2689220905303955
0.2604789137840271
0.29603469371795654

==> triangular_lax_hopf.tex <==
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.15906085073947906
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.738914430141449
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.1043429747223854
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.6108570694923401
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.22798000276088715
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.2919161319732666
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654

==> triangular_ours.tex <==
0.5
0.5113641023635864
0.5022833347320557
0.5101271867752075
0.5040627121925354
0.5070278644561768
0.5042788982391357
0.5049487948417664
0.5036898255348206
0.5034834742546082
0.50278639793396
0.5023424029350281
0.501835823059082
0.5013880133628845
0.500953197479248
0.5005698204040527
0.5001732110977173
0.49986496567726135
0.49948930740356445
0.49924784898757935
0.4988722503185272
0.49869024753570557
0.4982920289039612
0.49817749857902527
0.49773532152175903
0.497721791267395
0.4972083866596222
0.49735960364341736
0.4967220723628998
0.497140496969223
0.4962693154811859
0.4971183240413666
0.49579930305480957
0.49735352396965027
0.4952073395252228
0.4979556202888489
0.49419066309928894
0.49788734316825867
0.4907165467739105
0.46160468459129333
0.21230469644069672
0.13332849740982056
0.1475348174571991
0.12501974403858185
0.14267536997795105
0.1400136649608612
0.14100448787212372
0.14154323935508728
0.14093109965324402
0.14119952917099
0.1411077380180359
0.14063841104507446
0.1439966857433319
0.16070343554019928
0.761997640132904
0.8879415988922119
0.9003663063049316
0.8761740922927856
0.9117426872253418
0.8562098741531372
0.567302405834198
0.5044574737548828
0.5034917593002319
0.5003978610038757
0.5015855431556702
0.5001750588417053
0.5013866424560547
0.5003629326820374
0.5013075470924377
0.5007100701332092
0.5015465617179871
0.5013630390167236
0.5020125508308411
0.5018738508224487
0.502030074596405
0.501700758934021
0.5014505386352539
0.5010404586791992
0.5006090402603149
0.5002275109291077
0.49973759055137634
0.49943530559539795
0.49893102049827576
0.4987374544143677
0.49822038412094116
0.49816378951072693
0.4976043105125427
0.497724711894989
0.49706050753593445
0.4974285960197449
0.49655407667160034
0.4972977638244629
0.49603337049484253
0.49737927317619324
0.495415598154068
0.4977594017982483
0.4943222999572754
0.4973113238811493
0.49202242493629456
0.446579247713089
0.14229212701320648
0.06915390491485596
0.09167997539043427
0.06777475774288177
0.08556247502565384
0.0827791690826416
0.08321964740753174
0.08398056030273438
0.08336856961250305
0.08348025381565094
0.08364859223365784
0.08305114507675171
0.08601371943950653
0.08034256845712662
0.5834107398986816
0.8414794206619263
0.8429118990898132
0.8234591484069824
0.8590906262397766
0.803346574306488
0.5550243854522705
0.5049312710762024
0.5033966302871704
0.5010456442832947
0.5022042393684387
0.5008838176727295
0.5021359920501709
0.5010963082313538
0.5021187663078308
0.5014953017234802
0.5023751258850098
0.5021238327026367
0.5027034282684326
0.5024629235267639
0.5025361776351929
0.5021735429763794
0.5018995404243469
0.5015249252319336
0.5011094808578491
0.5008071064949036
0.500353217124939
0.5001645684242249
0.4997067451477051
0.4996594190597534
0.49919217824935913
0.49931102991104126
0.49879932403564453
0.4991121292114258
0.49849647283554077
0.49904072284698486
0.49824604392051697
0.4990725517272949
0.49802133440971375
0.4991859495639801
0.49782252311706543
0.49932917952537537
0.49747052788734436
0.4982888996601105
0.4951639175415039
0.4442940950393677
0.22244618833065033
0.2110167145729065
0.21785669028759003
0.20105530321598053
0.21772883832454681
0.2119034081697464
0.214072585105896
0.21388310194015503
0.21342667937278748
0.21386000514030457
0.21349717676639557
0.2138536423444748
0.21338580548763275
0.21406827867031097
0.21288663148880005
0.21443435549736023
0.21313214302062988
0.21467354893684387
0.21742142736911774
0.23500606417655945
0.28095221519470215
0.30298155546188354
0.29670262336730957
0.29827404022216797
0.2965310215950012
0.2956608235836029
0.29630225896835327
0.2958417534828186
0.29614776372909546
0.2958952784538269
0.29627472162246704
0.295585572719574
0.2966839075088501
0.294916570186615
0.29765912890434265
0.29567983746528625
0.30020055174827576
0.2990620732307434
0.2868608236312866
0.29603469371795654

==> underwood.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 0, 0, 0},
{0, -, 100, 100, 100, 0, 0, 0},
{0, 0, -, 100, 1, 0, 0, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 4, 100, -, 0, 0, 0},
{100, 100, 100, 100, 100, -, 0, 0},
{100, 100, 100, 100, 100, 100, -, 1},
{100, 100, 100, 100, 100, 100, 99, -},
}
